Weighted Sum-Rate Maximization for Movable Antenna-Enhanced Wireless Networks

This letter investigates the weighted sum rate maximization problem in movable antenna (MA)-enhanced systems. To reduce the computational complexity, we transform it into a more tractable weighted minimum mean square error (WMMSE) problem well-suited for MA. We then adopt the WMMSE algorithm and majorization-minimization algorithm to optimize the beamforming and antenna positions, respectively. Moreover, we propose a planar movement mode, which constrains each MA to a specified area, we obtain a low-complexity closed-form solution. Numerical results demonstrate that the MA-enhanced system outperforms the conventional system. Besides, the computation time for the planar movement mode is reduced by approximately 30\% at a little performance expense.

==> mathdef.tex <==

%
% Latex macro file
% File name: mathdef.tex
%

% Mathematical environments:
\def\BD{\begin{displaymath}}
\def\BE{\begin{equation}}
\def\BEA{\begin{eqnarray}}
\def\BEAs{\begin{eqnarray*}}
\def\ED{\end{displaymath}}
\def\EE{\end{equation}}
\def\EEA{\end{eqnarray}}
\def\EEAs{\end{eqnarray*}}

% Boldface Characters:
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
%\def\bf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bM{{\bf M}}
\def\bL{{\bf L}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bQ{{\bf Q}}
\def\bq{{\bf q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bt{{\bf t}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}

% Boldface greek:
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bDelta{\mbox{\boldmath $\Delta$}}
\def\beps{\mbox{\boldmath $\epsilon$}}
\def\b_eta{\mbox{\boldmath $\eta$}}
\def\bGamma{\mbox{\boldmath $\Gamma$}}
\def\bkappa{\mbox{\boldmath $\kappa$}}
\def\bLambda{\mbox{\boldmath $\Lambda$}}
\def\bnu{\mbox{\boldmat $\nu$}}
\def\bomega{\mbox{\boldmath $\omega$}}
\def\bPhi{\mbox{\boldmath $\Phi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{\mbox{\boldmath $\Psi$}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{\mbox{\boldmath $\Sigma$}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{\mbox{\boldmath $\Theta$}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bxi{\mbox{\boldmath $\xi$}}

% Caligraphy Characters:
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cL{{\cal L}}
\def\cP{{\cal P}}
\def\cR{{\cal R}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}

% Boldface caligraphy characters:
\def\bcA{\mbox{\boldmath ${\cal A}$}}

% Mathematical set characters:
\def\msC{{\Bbb C}}
\def\msI{{\Bbb I}}
\def\msR{{\Bbb R}}
\def\msZ{{\Bbb Z}}

% Frequently used operators:
\def\diag{{\rm diag}}
\def\dist{{\rm dist}}
\def\Imag{\mbox{Im}}
\def\Real{\mbox{Re}}
\def\trace{{\rm tr}}

% Useful abbreviations:
\def\eps{\epsilon}
\def\om{\omega}

% Others (to be fixed...)
\def\txi{{\tilde \xi}}
\def\ul{\underline}
\def\cspan{\mathop{\rm span} \nolimits}
%\def\Tr{{\rm tr}}
\def\sinc{{\rm sinc}}
\def\define{\buildrel \triangle \over =}
\def\spn{{\rm Span}}
\def \Cset    {\hbox{\hskip 2pt { I} \hskip -1.5pt \llap{C}}}
\def\bull{\vrule depth -.1ex
         width .8ex
         height .9ex}
\def\tvert{\vert \hskip -1pt \Vert}
\def\L2{L^{2}[-{\pi \over 2} , {\pi \over 2}]}
\def\integ{\int_{-{\pi \over 2}}^{{\pi \over 2}}}
\def\bnu{\bnu}
\def\ct{\hat{\btheta}}
\def\tk{\btheta^{k}}
\def\tki{\btheta^{k}_{i-1}}
\def\htk{\hat{\btheta}^{k}}
\def\htki{\hat{\btheta}^{k}_{i-1}}
\def\hR{\hat{\bf R}}
\def\brR{\bar{\bf R}}
\def\bRk{{\bf R}^{k}}
\def\hRk{\hat{{\bf R}}^{k}}
\def\hRki{\hat{{\bf R}}^{k}_{i-1}}
\def\Rki{{\bf R}^{k}_{i-1}}
\def\hs{\hat{\sigma}^{2}}
\def\hsk{\hat{\sigma}^{2}_{k}}
\def\hp{\hat{\psi}}
\def\RTCT{{\bf R}_{\rm TCT}}
\def\ECSM{{\cal E}_{\rm CSM}}
\def\ETCT{{\cal E}_{\rm TCT}}
\def\PCSM{\bPhi_{\rm CSM}}
\def\PTCT{\bPhi_{\rm TCT}}
\def\AIC{{\rm AIC}}
\def\MDL{{\rm MDL}}
\def\PSC{{\rm P\hspace{-.1em}S\hspace{-.1em}C}}
%\def\proof{{\bf Proof:}}
%\def\SNReq{{\rm SNR}_{eq}}
%\def\SNRth{{\rm SNR}_{th}}
%\def\mib{\bf}

